Towards Better Analysis of Machine Learning Models: A Visual Analytics Perspective

Interactive model analysis, the process of understanding, diagnosing, and refining a machine learning model with the help of interactive visualization, is very important for users to efficiently solve real-world artificial intelligence and data mining problems. Dramatic advances in big data analytics has led to a wide variety of interactive model analysis tasks. In this paper, we present a comprehensive analysis and interpretation of this rapidly developing area. Specifically, we classify the relevant work into three categories: understanding, diagnosis, and refinement. Each category is exemplified by recent influential work. Possible future research opportunities are also explored and discussed.

==> overview.tex <==
\section{Overview}

\begin{figure}
\centering
\includegraphics[width=\textwidth]{fig/MLPipeline}
\caption{An overview of interactive machine learning.}
\label{fig.ml_overview}
\end{figure}

\begin{figure}
\centering
\includegraphics[width=\textwidth]{fig/overview}
\caption{An overview of interactive model analysis.}
\end{figure} 
